Swarm-GPT: Combining Large Language Models with Safe Motion Planning for Robot Choreography Design

This paper presents Swarm-GPT, a system that integrates large language models (LLMs) with safe swarm motion planning - offering an automated and novel approach to deployable drone swarm choreography. Swarm-GPT enables users to automatically generate synchronized drone performances through natural language instructions. With an emphasis on safety and creativity, Swarm-GPT addresses a critical gap in the field of drone choreography by integrating the creative power of generative models with the effectiveness and safety of model-based planning algorithms. This goal is achieved by prompting the LLM to generate a unique set of waypoints based on extracted audio data. A trajectory planner processes these waypoints to guarantee collision-free and feasible motion. Results can be viewed in simulation prior to execution and modified through dynamic re-prompting. Sim-to-real transfer experiments demonstrate Swarm-GPT's ability to accurately replicate simulated drone trajectories, with a mean sim-to-real root mean square error (RMSE) of 28.7 mm. To date, Swarm-GPT has been successfully showcased at three live events, exemplifying safe real-world deployment of pre-trained models.

==> figures/figure_6_2d_combined.tex <==
\begin{groupplot}[group style={group size=3 by 1, horizontal sep=1em},
    width=7cm, height=7cm,
    ymin=-1.2, ymax=1.2, xmin=-1.2, xmax=1.2,
    ]
    \nextgroupplot[]
    \input{figures/figure_6_2d_part_1}
    \nextgroupplot[yticklabels={,,}]
    \input{figures/figure_6_2d_part_2}
    \nextgroupplot[yticklabels={,,}]
    \input{figures/figure_6_2d_part_3}
  \end{groupplot}


% \begin{groupplot}[group style={group size=3 by 1, horizontal sep=1em},
%     width=7cm, height=7cm,
%     ymin=-1.2, ymax=1.2, xmin=-1.2, xmax=1.2,
%     ]
%     \nextgroupplot[]
%     \input{figures/figure_6_2d}
%     \nextgroupplot[yticklabels={,,}]
%     \input{figures/figure_6_2d_2}
%     \nextgroupplot[yticklabels={,,}]
%     \input{figures/figure_6_2d_3}
%   \end{groupplot}

==> figures/figure_6_2d_part_1.tex <==
\addplot[only marks, blue!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9606237411499023 0.07670016586780548
};
\addplot[only marks, blue!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9669567942619324 0.1117405816912651
};
\addplot[only marks, blue!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9742741584777832 0.14536185562610626
};
\addplot[only marks, blue!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.983034074306488 0.1812644600868225
};
\addplot[only marks, blue!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9923459887504578 0.2159322053194046
};
\addplot[only marks, blue!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0023037195205688 0.25284621119499207
};
\addplot[only marks, blue!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0120903253555298 0.2876494824886322
};
\addplot[only marks, blue!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0200451612472534 0.31747865676879883
};
\addplot[only marks, blue!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0254522562026978 0.34530702233314514
};
\addplot[only marks, blue!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0265703201293945 0.3696412146091461
};
\addplot[only marks, blue!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0227454900741577 0.39072155952453613
};
\addplot[only marks, blue!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.012782335281372 0.4131585359573364
};
\addplot[only marks, blue!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9969183802604675 0.43736955523490906
};
\addplot[only marks, blue!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9766249060630798 0.4629973769187927
};
\addplot[only marks, blue!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9525133967399597 0.49225252866744995
};
\addplot[only marks, blue!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9203730821609497 0.529525101184845
};
\addplot[only marks, blue!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8896604180335999 0.5661998391151428
};
\addplot[only marks, blue!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8557494282722473 0.6080262064933777
};
\addplot[only marks, blue!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8216206431388855 0.6516658067703247
};
\addplot[only marks, blue!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7875254154205322 0.6965516209602356
};
\addplot[only marks, blue!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7558693289756775 0.7381524443626404
};

\addplot[only marks, green!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4495448172092438 0.8482125997543335
};
\addplot[only marks, green!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.41348493099212646 0.8419235348701477
};
\addplot[only marks, green!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.3740910291671753 0.8356451392173767
};
\addplot[only marks, green!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.3349098861217499 0.8300756216049194
};
\addplot[only marks, green!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.2968398630619049 0.8246721029281616
};
\addplot[only marks, green!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.2560514211654663 0.8190189003944397
};
\addplot[only marks, green!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.21888801455497742 0.8141432404518127
};
\addplot[only marks, green!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.18708699941635132 0.8098419904708862
};
\addplot[only marks, green!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.16216669976711273 0.8071686625480652
};
\addplot[only marks, green!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.14129406213760376 0.8050022721290588
};
\addplot[only marks, green!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.12698166072368622 0.8035516738891602
};
\addplot[only marks, green!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.1182987168431282 0.8028209805488586
};
\addplot[only marks, green!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.11155981570482254 0.8019117712974548
};
\addplot[only marks, green!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.10671921819448471 0.8008540272712708
};
\addplot[only marks, green!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.10240759700536728 0.7994885444641113
};
\addplot[only marks, green!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.09598828107118607 0.7971624732017517
};
\addplot[only marks, green!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.08928408473730087 0.794567346572876
};
\addplot[only marks, green!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.08103415369987488 0.7914373874664307
};
\addplot[only marks, green!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.07231234759092331 0.7882079482078552
};
\addplot[only marks, green!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.06223834678530693 0.7847793698310852
};
\addplot[only marks, green!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.053500715643167496 0.7820664644241333
};

\addplot[only marks, red!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.1675698608160019 -0.05098516866564751
};
\addplot[only marks, red!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.19647209346294403 -0.08378250151872635
};
\addplot[only marks, red!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.22776156663894653 -0.12134366482496262
};
\addplot[only marks, red!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2595401704311371 -0.16048336029052734
};
\addplot[only marks, red!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2898765504360199 -0.19825538992881775
};
\addplot[only marks, red!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3217633366584778 -0.2378745824098587
};
\addplot[only marks, red!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3524757921695709 -0.27486535906791687
};
\addplot[only marks, red!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3793158531188965 -0.30498063564300537
};
\addplot[only marks, red!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.40523993968963623 -0.3299518823623657
};
\addplot[only marks, red!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.42851078510284424 -0.3458675146102905
};
\addplot[only marks, red!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.44990888237953186 -0.3523145914077759
};
\addplot[only marks, red!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.47311514616012573 -0.3500201404094696
};
\addplot[only marks, red!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4980141520500183 -0.33906424045562744
};
\addplot[only marks, red!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5241791605949402 -0.32195010781288147
};
\addplot[only marks, red!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5536258220672607 -0.30010688304901123
};
\addplot[only marks, red!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5905709266662598 -0.271585613489151
};
\addplot[only marks, red!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6260327696800232 -0.24438029527664185
};
\addplot[only marks, red!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6657206416130066 -0.21549539268016815
};
\addplot[only marks, red!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7065114974975586 -0.18798744678497314
};
\addplot[only marks, red!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7482936382293701 -0.16156308352947235
};
\addplot[only marks, red!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7877976894378662 -0.13813020288944244
};

\addplot[only marks, cyan!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6379234194755554 -0.23429934680461884
};
\addplot[only marks, cyan!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.672968864440918 -0.2111726552248001
};
\addplot[only marks, cyan!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7068601250648499 -0.19098053872585297
};
\addplot[only marks, cyan!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7432229518890381 -0.17125746607780457
};
\addplot[only marks, cyan!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7784591317176819 -0.15350329875946045
};
\addplot[only marks, cyan!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8156614303588867 -0.13532935082912445
};
\addplot[only marks, cyan!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8506226539611816 -0.11804287135601044
};
\addplot[only marks, cyan!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.879474937915802 -0.10281521081924438
};
\addplot[only marks, cyan!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9042242169380188 -0.087761290371418
};
\addplot[only marks, cyan!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.922515332698822 -0.07268217951059341
};
\addplot[only marks, cyan!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9345813393592834 -0.0575701966881752
};
\addplot[only marks, cyan!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9429585933685303 -0.03909760341048241
};
\addplot[only marks, cyan!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9483065605163574 -0.01737136021256447
};
\addplot[only marks, cyan!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9527924656867981 0.006285055540502071
};
\addplot[only marks, cyan!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9571042060852051 0.033516090363264084
};
\addplot[only marks, cyan!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9627944231033325 0.06796467304229736
};
\addplot[only marks, cyan!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9696854948997498 0.10121189802885056
};
\addplot[only marks, cyan!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.978428065776825 0.13850699365139008
};
\addplot[only marks, cyan!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9884200692176819 0.17686177790164948
};
\addplot[only marks, cyan!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0003459453582764 0.2172841727733612
};
\addplot[only marks, cyan!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.011950135231018 0.25627216696739197
};

\addplot[only marks, magenta!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8873051404953003 0.5310656428337097
};
\addplot[only marks, magenta!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8585567474365234 0.5710173845291138
};
\addplot[only marks, magenta!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8309848308563232 0.6099403500556946
};
\addplot[only marks, magenta!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8016889691352844 0.651867687702179
};
\addplot[only marks, magenta!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7733931541442871 0.692503809928894
};
\addplot[only marks, magenta!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7431812882423401 0.7356814742088318
};
\addplot[only marks, magenta!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7144806981086731 0.7757564783096313
};
\addplot[only marks, magenta!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6900908946990967 0.8078828454017639
};
\addplot[only marks, magenta!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6676065325737 0.8329812288284302
};
\addplot[only marks, magenta!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6479204297065735 0.8469834923744202
};
\addplot[only marks, magenta!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6304256916046143 0.8491814136505127
};
\addplot[only marks, magenta!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6108868718147278 0.8400810956954956
};
\addplot[only marks, magenta!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5889745354652405 0.8206374645233154
};
\addplot[only marks, magenta!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5648901462554932 0.7947405576705933
};
\addplot[only marks, magenta!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5348726511001587 0.761216402053833
};
\addplot[only marks, magenta!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5004791617393494 0.7233576774597168
};
\addplot[only marks, magenta!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.46463045477867126 0.6856613159179688
};
\addplot[only marks, magenta!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.42448070645332336 0.6452730298042297
};
\addplot[only marks, magenta!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.38427698612213135 0.6060920357704163
};
\addplot[only marks, magenta!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3451427221298218 0.5694888234138489
};
\addplot[only marks, magenta!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.30933672189712524 0.5374912619590759
};

\addplot[only marks, yellow!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4474017918109894 0.6949779987335205
};
\addplot[only marks, yellow!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.41274747252464294 0.6591404676437378
};
\addplot[only marks, yellow!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3804904520511627 0.6260860562324524
};
\addplot[only marks, yellow!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3469398319721222 0.5928375720977783
};
\addplot[only marks, yellow!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3137472867965698 0.5605586767196655
};
\addplot[only marks, yellow!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.27762600779533386 0.5258353352546692
};
\addplot[only marks, yellow!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2424485683441162 0.491506963968277
};
\addplot[only marks, yellow!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2113928347826004 0.4596529006958008
};
\addplot[only marks, yellow!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.18735410273075104 0.4322175979614258
};
\addplot[only marks, yellow!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.16774924099445343 0.4043266773223877
};
\addplot[only marks, yellow!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.153922438621521 0.3774525225162506
};
\addplot[only marks, yellow!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.14267149567604065 0.3466407060623169
};
\addplot[only marks, yellow!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.13366621732711792 0.3117259442806244
};
\addplot[only marks, yellow!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.12501034140586853 0.271679550409317
};
\addplot[only marks, yellow!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.1165657490491867 0.22941002249717712
};
\addplot[only marks, yellow!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.10678722709417343 0.18005740642547607
};
\addplot[only marks, yellow!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.09714868664741516 0.12985225021839142
};
\addplot[only marks, yellow!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08619367331266403 0.07404232770204544
};
\addplot[only marks, yellow!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07578746229410172 0.01712437905371189
};
\addplot[only marks, yellow!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06519187241792679 -0.040081337094306946
};
\addplot[only marks, yellow!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.05549655109643936 -0.09306371957063675
};

==> figures/figure_6_2d_part_2.tex <==
\addplot[only marks, blue!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7558693289756775 0.7381524443626404
};
\addplot[only marks, blue!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7254575490951538 0.7779332399368286
};
\addplot[only marks, blue!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.695475161075592 0.814596951007843
};
\addplot[only marks, blue!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6682329773902893 0.8430295586585999
};
\addplot[only marks, blue!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6430235505104065 0.8609861135482788
};
\addplot[only marks, blue!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6194415092468262 0.8676233291625977
};
\addplot[only marks, blue!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5927913188934326 0.8636502623558044
};
\addplot[only marks, blue!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5628154873847961 0.849357545375824
};
\addplot[only marks, blue!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5303816199302673 0.8281568884849548
};
\addplot[only marks, blue!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.49161213636398315 0.7994494438171387
};
\addplot[only marks, blue!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.44878828525543213 0.7668222188949585
};
\addplot[only marks, blue!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4056466221809387 0.7347084879875183
};
\addplot[only marks, blue!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.35891374945640564 0.7009464502334595
};
\addplot[only marks, blue!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3122137784957886 0.669515073299408
};
\addplot[only marks, blue!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.26617300510406494 0.6410326957702637
};
\addplot[only marks, blue!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.22449274361133575 0.6167824864387512
};
\addplot[only marks, blue!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.18312528729438782 0.5942683815956116
};
\addplot[only marks, blue!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.14565053582191467 0.5756662487983704
};
\addplot[only marks, blue!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.1161704957485199 0.5617437362670898
};
\addplot[only marks, blue!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.09219972789287567 0.5501240491867065
};
\addplot[only marks, blue!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07677539438009262 0.5412405729293823
};
\addplot[only marks, green!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.053500715643167496 0.7820664644241333
};
\addplot[only marks, green!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.0438983291387558 0.779138445854187
};
\addplot[only marks, green!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.03284198045730591 0.7750486135482788
};
\addplot[only marks, green!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.02231440506875515 0.7691812515258789
};
\addplot[only marks, green!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.007877097465097904 0.7576248049736023
};
\addplot[only marks, green!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.009991103783249855 0.7394893169403076
};
\addplot[only marks, green!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.03567037358880043 0.7100433111190796
};
\addplot[only marks, green!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06855222582817078 0.6687303185462952
};
\addplot[only marks, green!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.10634948313236237 0.6189394593238831
};
\addplot[only marks, green!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.15233533084392548 0.5545129776000977
};
\addplot[only marks, green!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.20102304220199585 0.4800587296485901
};
\addplot[only marks, green!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.24754123389720917 0.40374425053596497
};
\addplot[only marks, green!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2949652075767517 0.31916144490242004
};
\addplot[only marks, green!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.33916446566581726 0.2335851490497589
};
\addplot[only marks, green!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3782166540622711 0.14982984960079193
};
\addplot[only marks, green!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.409555047750473 0.07376080006361008
};
\addplot[only marks, green!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4372105300426483 -0.00287623587064445
};
\addplot[only marks, green!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.45988523960113525 -0.07493223994970322
};
\addplot[only marks, green!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.47744864225387573 -0.1352398842573166
};
\addplot[only marks, green!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.49304455518722534 -0.18925133347511292
};
\addplot[only marks, green!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5064933896064758 -0.23115168511867523
};
\addplot[only marks, red!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7877976894378662 -0.13813020288944244
};
\addplot[only marks, red!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.826473593711853 -0.11606602370738983
};
\addplot[only marks, red!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8632571697235107 -0.09572707861661911
};
\addplot[only marks, red!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8936794400215149 -0.07780696451663971
};
\addplot[only marks, red!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9167918562889099 -0.06123785674571991
};
\addplot[only marks, red!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9321443438529968 -0.045201484113931656
};
\addplot[only marks, red!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9428863525390625 -0.02559923753142357
};
\addplot[only marks, red!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9495100378990173 -0.0016429678071290255
};
\addplot[only marks, red!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9542218446731567 0.025663752108812332
};
\addplot[only marks, red!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9585024118423462 0.0602341964840889
};
\addplot[only marks, red!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9633276462554932 0.09975910186767578
};
\addplot[only marks, red!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9692904353141785 0.1396562159061432
};
\addplot[only marks, red!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9765674471855164 0.18361960351467133
};
\addplot[only marks, red!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9850913882255554 0.2271927297115326
};
\addplot[only marks, red!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9944390058517456 0.2693522870540619
};
\addplot[only marks, red!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0031386613845825 0.30690252780914307
};
\addplot[only marks, red!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0122857093811035 0.34407585859298706
};
\addplot[only marks, red!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0202744007110596 0.3776232898235321
};
\addplot[only marks, red!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.027047038078308 0.4051383137702942
};
\addplot[only marks, red!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.032251000404358 0.4290759861469269
};
\addplot[only marks, red!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0343047380447388 0.44736653566360474
};
\addplot[only marks, cyan!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.011950135231018 0.25627216696739197
};
\addplot[only marks, cyan!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0235497951507568 0.29553595185279846
};
\addplot[only marks, cyan!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0331288576126099 0.3343365788459778
};
\addplot[only marks, cyan!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0384255647659302 0.36864981055259705
};
\addplot[only marks, cyan!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0377628803253174 0.3990092873573303
};
\addplot[only marks, cyan!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0302114486694336 0.4251784682273865
};
\addplot[only marks, cyan!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0147969722747803 0.45288562774658203
};
\addplot[only marks, cyan!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9919415712356567 0.4825606942176819
};
\addplot[only marks, cyan!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9646573662757874 0.5140454769134521
};
\addplot[only marks, cyan!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9308902025222778 0.5518864989280701
};
\addplot[only marks, cyan!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8937347531318665 0.5942401885986328
};
\addplot[only marks, cyan!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8569501638412476 0.6376742124557495
};
\addplot[only marks, cyan!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.817369818687439 0.6863426566123962
};
\addplot[only marks, cyan!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7783663272857666 0.7357910871505737
};
\addplot[only marks, cyan!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7409200072288513 0.7839720249176025
};
\addplot[only marks, cyan!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7074952125549316 0.8269200325012207
};
\addplot[only marks, cyan!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6748455166816711 0.8676469922065735
};
\addplot[only marks, cyan!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6452740430831909 0.9020451903343201
};
\addplot[only marks, cyan!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6221212148666382 0.9269753694534302
};
\addplot[only marks, cyan!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6019416451454163 0.9442760944366455
};
\addplot[only marks, cyan!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5871382355690002 0.9521012902259827
};
\addplot[only marks, magenta!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.30933672189712524 0.5374912619590759
};
\addplot[only marks, magenta!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.2743663489818573 0.507421612739563
};
\addplot[only marks, magenta!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.23940488696098328 0.4778164327144623
};
\addplot[only marks, magenta!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.20743326842784882 0.45034345984458923
};
\addplot[only marks, magenta!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.178863063454628 0.42408138513565063
};
\addplot[only marks, magenta!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.15495586395263672 0.3991070091724396
};
\addplot[only marks, magenta!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.1322450041770935 0.3710569441318512
};
\addplot[only marks, magenta!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.11240784823894501 0.34096911549568176
};
\addplot[only marks, magenta!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.09619465470314026 0.3106591999530792
};
\addplot[only marks, magenta!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08103255182504654 0.27669811248779297
};
\addplot[only marks, magenta!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06824895739555359 0.24162471294403076
};
\addplot[only marks, magenta!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.057641271501779556 0.20859560370445251
};
\addplot[only marks, magenta!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.0481267124414444 0.17454124987125397
};
\addplot[only marks, magenta!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.040078990161418915 0.1427401751279831
};
\addplot[only marks, magenta!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.033185917884111404 0.1141410619020462
};
\addplot[only marks, magenta!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.028618579730391502 0.08995285630226135
};
\addplot[only marks, magenta!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.024302590638399124 0.06807149946689606
};
\addplot[only marks, magenta!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.0202700924128294 0.04996620863676071
};
\addplot[only marks, magenta!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.01695162244141102 0.0359499491751194
};
\addplot[only marks, magenta!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.0125719690695405 0.024080494418740273
};
\addplot[only marks, magenta!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.007508095353841782 0.01453287061303854
};
\addplot[only marks, yellow!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.05549655109643936 -0.09306371957063675
};
\addplot[only marks, yellow!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.04543493688106537 -0.14783574640750885
};
\addplot[only marks, yellow!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.03661910817027092 -0.19514204561710358
};
\addplot[only marks, yellow!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.02732645906507969 -0.23908326029777527
};
\addplot[only marks, yellow!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.01725912280380726 -0.27521079778671265
};
\addplot[only marks, yellow!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.00576816825196147 -0.3020936846733093
};
\addplot[only marks, yellow!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.010160108096897602 -0.32384100556373596
};
\addplot[only marks, yellow!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.03139417618513107 -0.34025880694389343
};
\addplot[only marks, yellow!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.05768729746341705 -0.3522869646549225
};
\addplot[only marks, yellow!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.0912732183933258 -0.3636816442012787
};
\addplot[only marks, yellow!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.1301114857196808 -0.3747723400592804
};
\addplot[only marks, yellow!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.17014352977275848 -0.3863368332386017
};
\addplot[only marks, yellow!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.21406853199005127 -0.4000086188316345
};
\addplot[only marks, yellow!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.2581007182598114 -0.4152016341686249
};
\addplot[only marks, yellow!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.29981791973114014 -0.43136629462242126
};
\addplot[only marks, yellow!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.33697831630706787 -0.447334349155426
};
\addplot[only marks, yellow!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.372769832611084 -0.4644353985786438
};
\addplot[only marks, yellow!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4044269323348999 -0.48097914457321167
};
\addplot[only marks, yellow!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4286712408065796 -0.49497488141059875
};
\addplot[only marks, yellow!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4491332173347473 -0.5069345831871033
};
\addplot[only marks, yellow!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4639183282852173 -0.5143154859542847
};

==> figures/figure_6_2d_part_3.tex <==
\addplot[only marks, blue!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07677539438009262 0.5412405729293823
};
\addplot[only marks, blue!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06792780011892319 0.5326840281486511
};
\addplot[only marks, blue!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06488021463155746 0.5238747596740723
};
\addplot[only marks, blue!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06683456897735596 0.5138968825340271
};
\addplot[only marks, blue!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07212948799133301 0.500004231929779
};
\addplot[only marks, blue!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07837722450494766 0.4824002981185913
};
\addplot[only marks, blue!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08397305756807327 0.460618257522583
};
\addplot[only marks, blue!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08763431012630463 0.4364404082298279
};
\addplot[only marks, blue!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08918191492557526 0.40709835290908813
};
\addplot[only marks, blue!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.0878109261393547 0.37500083446502686
};
\addplot[only marks, blue!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.08473998308181763 0.3430415093898773
};
\addplot[only marks, blue!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07898054271936417 0.3079225718975067
};
\addplot[only marks, blue!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.07191581279039383 0.2707180976867676
};
\addplot[only marks, blue!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.06388681381940842 0.23470650613307953
};
\addplot[only marks, blue!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.05529716983437538 0.1980644315481186
};
\addplot[only marks, blue!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.047257717698812485 0.1668398678302765
};
\addplot[only marks, blue!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.03892570734024048 0.13879239559173584
};
\addplot[only marks, blue!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.03019651584327221 0.11608331650495529
};
\addplot[only marks, blue!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.02113143354654312 0.09825077652931213
};
\addplot[only marks, blue!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.008849828504025936 0.08180362731218338
};
\addplot[only marks, blue!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.006610256154090166 0.06577461957931519
};
\addplot[only marks, green!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5064933896064758 -0.23115168511867523
};
\addplot[only marks, green!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.519429624080658 -0.25947290658950806
};
\addplot[only marks, green!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5344831943511963 -0.2783147990703583
};
\addplot[only marks, green!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5519521236419678 -0.28701719641685486
};
\addplot[only marks, green!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5714032649993896 -0.2877368628978729
};
\addplot[only marks, green!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5953369736671448 -0.28225407004356384
};
\addplot[only marks, green!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6223206520080566 -0.27200061082839966
};
\addplot[only marks, green!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6498090624809265 -0.2594744861125946
};
\addplot[only marks, green!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6806394457817078 -0.24434439837932587
};
\addplot[only marks, green!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7115797400474548 -0.22837865352630615
};
\addplot[only marks, green!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7400825619697571 -0.21326835453510284
};
\addplot[only marks, green!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7701143026351929 -0.19750067591667175
};
\addplot[only marks, green!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8005266785621643 -0.18112871050834656
};
\addplot[only marks, green!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8293972611427307 -0.16519685089588165
};
\addplot[only marks, green!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8589543104171753 -0.14857058227062225
};
\addplot[only marks, green!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8854990601539612 -0.13306164741516113
};
\addplot[only marks, green!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.906208872795105 -0.11975494027137756
};
\addplot[only marks, green!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9230000376701355 -0.10671874135732651
};
\addplot[only marks, green!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9342676997184753 -0.09462466090917587
};
\addplot[only marks, green!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9426321983337402 -0.08116065710783005
};
\addplot[only marks, green!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9479584693908691 -0.06560668349266052
};
\addplot[only marks, red!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0343047380447388 0.44736653566360474
};
\addplot[only marks, red!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0326193571090698 0.4632973372936249
};
\addplot[only marks, red!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.027046799659729 0.477562814950943
};
\addplot[only marks, red!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0176254510879517 0.4912188947200775
};
\addplot[only marks, red!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-1.0025733709335327 0.5075780749320984
};
\addplot[only marks, red!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9837491512298584 0.5274273753166199
};
\addplot[only marks, red!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9613311886787415 0.5516951084136963
};
\addplot[only marks, red!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.9365414381027222 0.578192412853241
};
\addplot[only marks, red!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.908441960811615 0.6100031733512878
};
\addplot[only marks, red!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8785540461540222 0.6445817947387695
};
\addplot[only marks, red!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8500350117683411 0.678490400314331
};
\addplot[only marks, red!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.8191413283348083 0.7151066660881042
};
\addplot[only marks, red!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7872083783149719 0.7529999017715454
};
\addplot[only marks, red!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7569426894187927 0.7888226509094238
};
\addplot[only marks, red!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7261852622032166 0.82469642162323
};
\addplot[only marks, red!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.7002294659614563 0.8540989756584167
};
\addplot[only marks, red!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6767560839653015 0.878315806388855
};
\addplot[only marks, red!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6567783951759338 0.8940209150314331
};
\addplot[only marks, red!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6409346461296082 0.9001911878585815
};
\addplot[only marks, red!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6250727772712708 0.8980376720428467
};
\addplot[only marks, red!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.6085039973258972 0.8877211809158325
};
\addplot[only marks, cyan!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5871382355690002 0.9521012902259827
};
\addplot[only marks, cyan!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5747426152229309 0.9519199132919312
};
\addplot[only marks, cyan!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5636265277862549 0.9442223906517029
};
\addplot[only marks, cyan!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5526120066642761 0.9315260648727417
};
\addplot[only marks, cyan!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.538826584815979 0.9135395288467407
};
\addplot[only marks, cyan!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.5214748382568359 0.8928006291389465
};
\addplot[only marks, cyan!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4998568892478943 0.8706294298171997
};
\addplot[only marks, cyan!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.47513097524642944 0.8490371704101562
};
\addplot[only marks, cyan!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.4451753497123718 0.8259681463241577
};
\addplot[only marks, cyan!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.41242724657058716 0.802930474281311
};
\addplot[only marks, cyan!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3794914484024048 0.7814575433731079
};
\addplot[only marks, cyan!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3443203270435333 0.7585572004318237
};
\addplot[only marks, cyan!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.3078659474849701 0.7347329258918762
};
\addplot[only marks, cyan!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.273637980222702 0.7114607095718384
};
\addplot[only marks, cyan!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.23971128463745117 0.6870032548904419
};
\addplot[only marks, cyan!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.21201059222221375 0.6649794578552246
};
\addplot[only marks, cyan!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.1881578415632248 0.6436365842819214
};
\addplot[only marks, cyan!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.17130552232265472 0.6241247653961182
};
\addplot[only marks, cyan!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.16121679544448853 0.607151448726654
};
\addplot[only marks, cyan!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.15549494326114655 0.5896250009536743
};
\addplot[only marks, cyan!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.15273895859718323 0.5715456604957581
};
\addplot[only marks, magenta!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
-0.007508095353841782 0.01453287061303854
};
\addplot[only marks, magenta!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.00026206739130429924 0.005022921599447727
};
\addplot[only marks, magenta!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.010912706144154072 -0.005682591814547777
};
\addplot[only marks, magenta!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.025124501436948776 -0.01895645074546337
};
\addplot[only marks, magenta!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.042125534266233444 -0.03483644127845764
};
\addplot[only marks, magenta!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.06410109996795654 -0.05559526011347771
};
\addplot[only marks, magenta!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.08916951715946198 -0.08000867068767548
};
\addplot[only marks, magenta!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.1154569685459137 -0.10548664629459381
};
\addplot[only marks, magenta!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.14488480985164642 -0.13440002501010895
};
\addplot[only marks, magenta!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.17543350160121918 -0.164118692278862
};
\addplot[only marks, magenta!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.20434869825839996 -0.19227929413318634
};
\addplot[only marks, magenta!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.2349356710910797 -0.2218184918165207
};
\addplot[only marks, magenta!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.26682090759277344 -0.2526567578315735
};
\addplot[only marks, magenta!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.296964555978775 -0.2825581133365631
};
\addplot[only marks, magenta!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.32820138335227966 -0.31336864829063416
};
\addplot[only marks, magenta!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.355179101228714 -0.3394140899181366
};
\addplot[only marks, magenta!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.37945234775543213 -0.36188387870788574
};
\addplot[only marks, magenta!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.39975705742836 -0.3773166835308075
};
\addplot[only marks, magenta!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4159291088581085 -0.3848826289176941
};
\addplot[only marks, magenta!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4318799078464508 -0.3854629099369049
};
\addplot[only marks, magenta!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.44867050647735596 -0.3790621757507324
};
\addplot[only marks, yellow!10!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4639183282852173 -0.5143154859542847
};
\addplot[only marks, yellow!14!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.47636348009109497 -0.5174039006233215
};
\addplot[only marks, yellow!19!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.4878808259963989 -0.5144616961479187
};
\addplot[only marks, yellow!23!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.5007205605506897 -0.5056557059288025
};
\addplot[only marks, yellow!28!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.5152170658111572 -0.4918523132801056
};
\addplot[only marks, yellow!32!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.5350192189216614 -0.47178012132644653
};
\addplot[only marks, yellow!37!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.5588852763175964 -0.44765329360961914
};
\addplot[only marks, yellow!41!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.585541307926178 -0.42215099930763245
};
\addplot[only marks, yellow!46!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.6173698902130127 -0.3931710124015808
};
\addplot[only marks, yellow!50!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.6518775820732117 -0.36365434527397156
};
\addplot[only marks, yellow!55!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.6856022477149963 -0.3361791968345642
};
\addplot[only marks, yellow!59!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.7220250368118286 -0.30723604559898376
};
\addplot[only marks, yellow!64!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.7594865560531616 -0.2775619626045227
};
\addplot[only marks, yellow!68!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.7947500348091125 -0.24891801178455353
};
\addplot[only marks, yellow!73!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.8302861452102661 -0.21989692747592926
};
\addplot[only marks, yellow!77!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.8598297834396362 -0.19542524218559265
};
\addplot[only marks, yellow!82!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.885444164276123 -0.1734100878238678
};
\addplot[only marks, yellow!86!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.9044772386550903 -0.15546151995658875
};
\addplot[only marks, yellow!91!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.9170953631401062 -0.1407618522644043
};
\addplot[only marks, yellow!95!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.9255684018135071 -0.12560397386550903
};
\addplot[only marks, yellow!100!white, mark=*, mark size=3, fill opacity = 0.5] table 
{
0.9301518201828003 -0.10911351442337036
};
